Adaptive and quasi-sliding control of shimmy in landing gears

Shimmy is a dangerous phenomenon that occurs when aircraft's nose landing gears oscillate in a rapid and uncontrollable fashion. In this paper, we propose the use of two nonlinear control approaches (zero average control and model reference adaptive control based on minimal control synthesis) as simple yet effective strategies to suppress undesired oscillations, even in the presence of uncertainties and partial state measurements. Numerical results are presented to validate the proposed control approaches.

==> aux_file.tex <==


A common problem regarding airplanes' takeoff and landing is the possibility of the onset of violent oscillations of the nose landing gear (NLG).
This phenomenon, also known as \emph{shimmy}, is highly dangerous if not properly addressed, as it can make the aircraft uncontrollable by the pilot and lead to disastrous accidents.

In general, shimmy can happen in all those settings where an elastic wheel is rotating in contact with the ground and can steer around a vertical axis.
In fact, motorcycles are another relevant example of vehicles subject to this problem, which is also called \emph{wobble} in the field \cite{cossalter2006, limebeer2006}.

As a consequence of the diffusion and the practical meaningfulness of shimmy, it has been studied since the first tires were manufactured, up until now \cite{somieski1997, bonfe2011, takacs2009, takacs2010}.


Nevertheless, both from a theoretical and a technological point of view, there is still room for improvement.
To show this, we will focus on the recent work by Pouly et al. \cite{pouly2011}, and illustrate how the results in our work compare to those in the cited paper.
Namely, in \cite{pouly2011}, a rather sophisticated control scheme is employed, that involves a feedback linearization in combination with a fuzzy logic component, which is used to estimate the nonlinear part of the model to be compensated.
However, we found that simpler control strategies can achieve equal or better results.
For example, we propose the use of a model reference adaptive control (MRAC) with model control synthesis (MCS) and a zero average dynamics (ZAD), to achieve comparable outcomes.
In addition, all of the above control schemes require the knowledge of the whole state of the system.
However, as noted e.g. in \cite{bonfe2011}, this is not easily doable in practice for two reasons: either when cost minimization is a priority and the least number of sensors is installed, or when high reliability requires redundancy of sensors and again it is preferred to not measure all the state variables as this would imply a too large number of sensors.
To make up for the lack of the full array of sensors, we developed a state observer.
Moreover, in practice, it is not uncommon that the mathematical model of the NLG  is not completely adherent to its real dynamics, either because some parameters are not precisely estimated or because the very forms of some functions in the model are not representative enough.
To account for this issue, we use a modeling for the control synthesis and the observer design and a different one for the simulation of the NLG. 
This way, we create a model uncertainty, which, as we will show, is managed well by the control schemes we implemented.

The rest of the paper is outlined as follow.
In Section \ref{sec:Problem Statement}, we illustrate the problem in its mathematical formulation and define the control goals.
In particular, we present two different modelings describing the shimmy phenomenon and the relative bifurcation diagram with respect to the vehicle linear velocity.
Next, in Section \ref{sec:Controlling Shimmy}, we introduce the two control strategies that we use to tame shimmy, namely the MCS and the ZAD.
After that, Section \ref{sec:Numerical Results} contains the numerical results of the simulations of two different scenarios: one representing a tire damage and the other one representing a taxiing on a non-uniform road.
Finally, In Section \ref{sec:Conclusions}, we summarize the concepts and result exposed and give a series of considerations.
